DZip: improved general-purpose lossless compression based on novel neural network modeling

We consider lossless compression based on statistical data modeling followed by prediction-based encoding, where an accurate statistical model for the input data leads to substantial improvements in compression. We propose DZip, a general-purpose compressor for sequential data that exploits the well-known modeling capabilities of neural networks (NNs) for prediction, followed by arithmetic coding. Dzip uses a novel hybrid architecture based on adaptive and semi-adaptive training. Unlike most NN based compressors, DZip does not require additional training data and is not restricted to specific data types, only needing the alphabet size of the input data. The proposed compressor outperforms general-purpose compressors such as Gzip (on average 26% reduction) on a variety of real datasets, achieves near-optimal compression on synthetic datasets, and performs close to specialized compressors for large sequence lengths, without any human input. The main limitation of DZip in its current implementation is the encoding/decoding time, which limits its practicality. Nevertheless, the results showcase the potential of developing improved general-purpose compressors based on neural networks and hybrid modeling.

==> DZip IEEETran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> DZip IEEETran/dataset_table.tex <==
% \begin{table*}[!htbp]
% 	\centering
% 	\caption{Real and synthetic datasets used for evaluation. {$|\mathcal{S}|$} denotes the alphabet size. (bpc stands for bits per character)}
% 	\label{table:data}
% 	\vskip 0.15in
% 	\begin{small}
% 		\begin{tabular}{llll}
% 			\hline
% 			\textbf{Name}     & \textbf{Length} & {$|\mathcal{S}|$} & \textbf{Description} \\ 
% 			\hline
% 			\textbf{Real Datasets} & & &\\
% 			\hline
% 			\emph{webster}& 41.1M & 98 & HTML data of the 1913 Webster Dictionary, from the Silesia corpus \\
% 			\emph{mozilla}& 51.2M & 256 & Tarred executables of Mozilla 1.0, from the Silesia corpus\\
% 			\emph{h.\ chr20} & 64.4M & 5 &  Chromosome 20 of \emph{H. sapiens} GRCh38 reference sequence %\cite{hgenome}
% 			\\
% 			\emph{h.\ chr1} & 100M & 5 & First 100M bases of chromosome 1 of \emph{H. Sapiens} GRCh38 sequence%\cite{hgenome}\\%\cite{hgp}  \\
% 			\\
% 			\emph{c.e.\ genome}  & 100M & 4 & \textit{C.\ elegans} whole genome sequence\\
% 			\emph{ill-quality}& 100M & 4 & 100MB of quality scores for PhiX virus reads sequenced with Illumina \\
% 			\emph{text8} & 100M & 27 &  First 100M of English text (only) extracted from \emph{enwiki9}\\
% 			\emph{np-bases}&  300M & 5 & Nanopore sequenced reads (only bases) of a human sample truncated to 300M symbols \\
% 			\emph{np-quality}& 300M & 91 & Quality scores for nanopore sequenced data of a human sample truncated to 300M symbols\\
% 			\emph{enwiki9}&  500M & 206 & First 500M of the English Wikipedia dump on 2006\\
% 			\emph{num-control}&  159.5M & 256 & Control vector output between two minimization steps in weather-satellite data assimilation\\
% 			\emph{obs-spitzer}&  198.2M & 256 & Data from the Spitzer Space Telescope showing a slight darkening\\
% 			\emph{msg-bt}&  266.4M & 256 & NPB computational fluid dynamics pseudo-application bt\\
% 			\emph{audio}&  264.6M & 256 & First 600 files (combined) in ESC Dataset for environmental sound classification\\
% 			& & & [\url{https://github.com/karolpiczak/ESC-50}]\\
% 			\hline
% 			\textbf{Synthetic Datasets} & & &\\
% 			\hline
% 			\emph{XOR-k}  & 10M & 2 & Pseudorandom sequence $S_{n+1} = S_n + S_{n-k}\ (\textnormal{mod}\ 2)$ . Entropy rate $0$ bpc. [\citet{knuth2014art}]\\
% 			\emph{HMM-k} & 10M & 2 & Hidden Markov sequence $S_n = X_n + Z_n\ (\textnormal{mod}\ 2)$, with $Z_n \sim Bern(0.1)$,\\
% 			& & & $X_{n+1} = X_n + X_{n-k}\ (\textnormal{mod}\ 2)$. Entropy rate $0.46899$ bpc.\\
% 			\hline
% 	\end{tabular}
% 	\end{small}
% \end{table*}  


\begin{table*}[!htbp]
	\centering
	\caption{Real and synthetic datasets used for evaluation. {$|\mathcal{S}|$} denotes the alphabet size. bpc stands for bits per character. %\blue{Links to all the datasets are available on our github repository (\url{https://github.com/mohit1997/Dzip-torch}).}
	}
	\label{table:data}
	\vskip 0.15in
	\begin{small}
		\begin{tabular}{llll}
			\hline
			\textbf{Name}     & \textbf{Length} & {$|\mathcal{S}|$} & \textbf{Description} \\ 
			\hline
			\textbf{Real Datasets} & & &\\
			\hline
			
			a) Text & & &\\
			\hline
			\emph{webster}& 41.1M & 98 & HTML data of the 1913 Webster Dictionary, from the Silesia corpus \\
			\emph{text8} & 100M & 27 &  First 100M of English text (only) extracted from \emph{enwiki9}\\
			\emph{enwiki9}&  500M & 206 & First 500M of the English Wikipedia dump on 2006\\
			\hline
			
			b) Executables  & & &\\
			\hline
			\emph{mozilla}& 51.2M & 256 & Tarred executables of Mozilla 1.0, from the Silesia corpus\\
			\emph{h.\ chr20} & 64.4M & 5 &  Chromosome 20 of \emph{H. sapiens} GRCh38 reference sequence %\cite{hgenome}
			\\
			\hline
			c) Genomic Data & & &\\
			\hline
			\emph{h.\ chr1} & 100M & 5 & First 100M bases of chromosome 1 of \emph{H. Sapiens} GRCh38 sequence%\cite{hgenome}\\%\cite{hgp}  \\
			\\
			\emph{c.e.\ genome}  & 100M & 4 & \textit{C.\ elegans} whole genome sequence\\
			\emph{ill-quality}& 100M & 4 & 100MB of quality scores for PhiX virus reads sequenced with Illumina \\
			
			\emph{np-bases}&  300M & 5 & Nanopore sequenced reads (only bases) of a human sample (first 300M symbols) \\
			\emph{np-quality}& 300M & 91 & Quality scores for nanopore sequenced human sample (first 300M symbols)\\
			\hline
			d) Floating Point & &\\
			\hline
			\emph{num-control}&  159.5M & 256 & Control vector output between two minimization steps in weather-satellite data assimilation\\
			\emph{obs-spitzer}&  198.2M & 256 & Data from the Spitzer Space Telescope showing a slight darkening\\
			\emph{msg-bt}&  266.4M & 256 & NPB computational fluid dynamics pseudo-application bt\\
			\hline
			
			e) Audio (wav) & & &\\
			\hline
			\emph{audio}&  264.6M & 256 & First 600 files (combined) in ESC Dataset for environmental sound classification \\
% 			& & & [\url{https://github.com/karolpiczak/ESC-50}]\blue{[IO: only one with link...]}\\
			\hline
			\textbf{Synthetic Datasets} & & &\\
			\hline
			\emph{XOR-k}  & 10M & 2 & Pseudorandom sequence $S_{n+1} = S_n + S_{n-k}\ (\textnormal{mod}\ 2)$. \\
			&&& Entropy rate $0$ bpc.\\
			\emph{HMM-k} & 10M & 2 & Hidden Markov sequence $S_n = X_n + Z_n\ (\textnormal{mod}\ 2)$, with $Z_n \sim Bern(0.1)$,\\
			& & & $X_{n+1} = X_n + X_{n-k}\ (\textnormal{mod}\ 2)$. Entropy rate $0.46899$ bpc. \\
			\hline
	\end{tabular}
	\end{small}
\end{table*}  


==> DZip IEEETran/results_comparison.tex <==
% \begin{table}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{File}}     & \multirow{2}{*}{\textbf{Length}} & \textbf{Bootstrap}  & \textbf{Randomly initialized} & \textbf{DZip} \\ 
%      &  & \textbf{only}  & \textbf{combined model} & \textbf{(hybrid)} \\ \hline
% \textit{webster}  & 41.1M & 0.994 & 1.126 & 0.943   \\ \hline
% \textit{mozilla}  & 51.2M & 1.680 & 1.860 & 1.630   \\ \hline
% \textit{H. chr20} & 64.4M & 1.657 & 1.630 & 1.614 \\ \hline
% \end{tabular}
% \caption{Comparing bits per character \red{(only arithmetic coding output)} for three scenarios. }
% \label{table:results_comparison}
% \end{table}

\begin{table}[!htbp]
\centering
\caption{Compression in bpc obtained by (i) only the bootstrap model and (ii) DZip (combined model). Improv. stands for the improvement of the combined model with respect to the bootstrap model (in bpc).}
\label{table:results_comparison}
\vskip 0.15in
\begin{small}
\begin{sc}

\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{\textbf{File}}     & \multirow{2}{*}{\textbf{Length}} & \textbf{Bootstrap}  & \multirow{2}{*}{\textbf{DZip}} & \multirow{1}{*}{\textbf{Improv.}} \\ 
     &  & \textbf{only} & & \textbf{(bpc)}\\ \midrule
\textit{webster}  & 41.1M & 1.474 &  1.443  & 0.031 \\ 
\textit{mozilla}  & 51.2M & 2.233 &  2.150  & 0.083 \\ 
\textit{h. chr20} & 64.4M & 1.672 &  1.634 & 0.038\\ 
\textit{h. chr1} & 100M & 1.720 & 1.673 & 0.047\\ 
\textit{c.e. genome} & 100M & 1.826 &  1.814 & 0.012\\ 
\textit{ill-quality} & 100M & 0.343 & 0.343 & 0.000 \\ 
\textit{text8} & 100M & 1.789 & 1.737 & 0.052\\ 
\textit{np-bases} & 300M & 1.755 & 1.725 &0.03\\ 
\textit{np-quality} & 300M & 5.588 & 5.562 & 0.026\\ 
\textit{enwiki9} & 500M & 1.596 & 1.470 &0.126\\
\textit{num-control} & 159.5M & 6.838 & 6.834 &0.004\\
\textit{obs-spitzer} & 198.2M & 2.445 & 2.181 &0.264\\
\textit{msg-bt} & 266.4M & 5.259 & 5.214 &0.045\\
\textit{audio} & 264.6M & 3.405 & 3.389 &0.016\\\midrule
\textit{XOR-30} & 10M & 0.011 & 0.011 & 0.0\\ 
\textit{HMM-30} & 10M & 0.482 & 0.482 & 0.0\\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}

==> DZip IEEETran/results_real_data.tex <==
% \begin{table*}[!htbp]
% \centering
% \caption{Bits per character (bpc) achieved by the tested compressors on the real datasets. Best results are boldfaced. $\log_2|\mathcal{S}|$ represents the bpc achieved assuming an independent uniform distribution over the alphabet of size $|\mathcal{S}|$. For DZip, we specify the total bpc and the size of the model (in \% space occupied). Spec. Comp. stands for specialized compressor. %refers to the specialized compressors. the bpc achieved by the specialized compressors: ZPAQ (webster, text8, enwiki9); GeCo (H. Chr20, H. Chr1, C.E. Gen, NP Bases); and QVZ (Ill Qual.).
% }
% \label{table:results_real}
% \vskip 0.15in
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccccccc|cc|c}
% \toprule
% \multirow{2}{*}{\textbf{File}} & \multirow{2}{*}{\textbf{Len/$\mathbf{log_2|\mathcal{S}|}$}} & \multirow{2}{*}{\textbf{Gzip}} & \multicolumn{1}{c}{\textbf{LSTM}} & \multirow{2}{*}{\textbf{BSC}} & \multirow{2}{*}{\textbf{7zip}} & \multirow{2}{*}{\textbf{ZPAQ}} & \multirow{2}{*}{\textbf{NNCP}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{CMIX}}} & \multicolumn{2}{c|}{\textbf{DZip}}                                                           & \multirow{1}{*}{\textbf{Spec.}} \\ \cline{10-11}
%                               &                                     &                                & \multicolumn{1}{c}{\textbf{Compress}}                               & & & & & \multicolumn{1}{l|}{}                              & \multicolumn{1}{c|}{\textbf{bpc}} & \multicolumn{1}{l|}{\textbf{Model}} &  \multirow{1}{*}{\textbf{Comp.}}                               \\ \midrule
% \textit{webster}               & 41.1M/6.61                            & 2.32                           & 1.23                                       & 1.29             & 1.70  & 1.09  &   0.98  &   \textbf{0.83}                         & 1.44                                & 31.33\%                                  & 0.83                            \\
% \textit{mozilla}               & 51.2M/8.00                           & 2.97                           & 2.05                                     & 2.52                & 2.11   & 1.88 &  1.63  &   \textbf{1.39}                         & 2.15                                & 25.37\%                                & 1.39                              \\
% \textit{h.\ chr20}              & 64.4M/2.32                             & 2.05                           & 7.82                                                & 1.73             & 1.77  &    1.68    & 1.66    &    \textbf{1.62}                     & 1.63                       & 0.92\%                                  & 1.62                            \\
% \textit{h.\ chr1}               & 100M/2.32                            & 2.14                           & 7.36                                                & 1.78         & 1.83 &   1.74   &   \textbf{1.67}  &       \textbf{1.67}                         & \textbf{1.67}                       & 0.58\%                                  & 1.65                            \\
% \textit{c.e.\ genome}              & 100M/2.00                              & 2.15                           & 7.51                                                & 1.87         & 1.89    &  1.80   &  1.80   &     \textbf{1.74}                          & 1.81                       & 0.53\%                                 & 1.72                            \\
% \textit{ill-quality}             & 100M/2.00                              & 0.50                           & 6.48                                                & 0.35          & 0.35      & 0.34  &   0.34  &    \textbf{0.33}                         & 0.34                       & 2.79\%                                   & 0.51                            \\
% \textit{text8}                 & 100M/4.75                             & 2.64                           & 1.76                                                & 1.68        & 1.93  &  1.52  &  1.48   &    \textbf{1.31}                     & 1.74                                & 9.38\%                                      & 1.31                            \\
% \textit{np-bases}              & 300M/2.32                              & 2.16                           & 7.34                                                & 1.86               & 1.93 &  1.79   &   \textbf{1.70}  &      1.73                       & 1.73                       & 0.19\%                                 & 1.75                            \\
% \textit{np-quality}              & 300M/6.51                             & 5.95                           & 5.51                                                & 5.69     & 5.71   & 5.53    &   5.50  &     \textbf{5.49}                                & 5.56                       & 1.13\%                                  & 5.35                             \\ 
% \textit{enwiki9}               & 500M/7.69                            & 2.72                           & 1.66                                                & 1.64    & 1.94        &     1.43         &   1.21  &    \textbf{1.05}                    & 1.47                       & 3.67\%                                     & 1.05                            \\


% \textit{num-control}               & 159.5M/7.69                            & 7.57                           & 6.82                                                & 7.66    & 7.41     &   6.96               &   6.72  &    \textbf{6.63}                    & 6.83                 & 2.67\%                                     & 7.12                            \\
% \textit{obs-spitzer}               & 198.2M/7.69                            & 6.50                           & 2.87                                                & 2.51   & 2.27      &     2.20            &   1.73  &    \textbf{1.58}                   & 2.18                 & 6.70\%                                     & 7.74                            \\
% \textit{msg-bt}               & 266.4M/7.69                            & 7.08                           & 6.22                                                & 6.96     & 5.76          &    6.29        &   5.361  &    5.24                    & \textbf{5.21}                       & 2.08\%                                     & 6.67                            \\
% \textit{audio}               & 264.6M/7.69                            & 5.75                           & 4.92                                                & 4.63   &   4.98           &    4.17     &   3.49  &    3.50                    & \textbf{3.40}                       & 3.29\%                                     & N/A                            \\\bottomrule
% \end{tabular}
% \end{sc}
% \end{small}

% \end{table*}


\begin{table*}[!htbp]
\centering
\caption{Bits per character (bpc) achieved by the tested compressors on the real datasets. Best results are boldfaced. $\log_2|\mathcal{S}|$ represents the bpc achieved assuming an independent uniform distribution over the alphabet of size $|\mathcal{S}|$. For DZip, we specify the total bpc and the size of the model (in \% space occupied). Spec. Comp. stands for specialized compressor. %refers to the specialized compressors. the bpc achieved by the specialized compressors: ZPAQ (webster, text8, enwiki9); GeCo (H. Chr20, H. Chr1, C.E. Gen, NP Bases); and QVZ (Ill Qual.).
}
\label{table:results_real}
\vskip 0.15in
\begin{small}
\begin{sc}
\begin{tabular}{ccccccccc|cc|c}
\toprule
\multirow{2}{*}{\textbf{File}} & \multirow{2}{*}{\textbf{Len/$\mathbf{log_2|\mathcal{S}|}$}} & \multirow{2}{*}{\textbf{Gzip}} & \multirow{2}{*}{\textbf{BSC}} & \multirow{2}{*}{\textbf{7zip}} & \multirow{2}{*}{\textbf{ZPAQ}} & \multicolumn{1}{c}{\textbf{LSTM}}  & \multirow{2}{*}{\textbf{NNCP}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{CMIX}}} & \multicolumn{2}{c|}{\textbf{DZip}}                                                           & \multirow{1}{*}{\textbf{Spec.}} \\ \cline{10-11}
                               &                                     &                                                               & & & & \multicolumn{1}{c}{\textbf{Compress}} & & \multicolumn{1}{l|}{}                              & \multicolumn{1}{c|}{\textbf{bpc}} & \multicolumn{1}{l|}{\textbf{Model}} &  \multirow{1}{*}{\textbf{Comp.}}                               \\ \midrule
\textit{webster}               & 41.1M/6.61                            & 2.32                                                                 & 1.29             & 1.70  & 1.09   & 1.23 &   0.98  &   \textbf{0.83}                         & 1.44                                & 31.33\%                                  & 0.83                            \\
\textit{mozilla}               & 51.2M/8.00                           & 2.97                                                                & 2.52                & 2.11   & 1.88 & 2.05 &  1.63  &   \textbf{1.39}                         & 2.15                                & 25.37\%                                & 1.39                              \\
\textit{h.\ chr20}              & 64.4M/2.32                             & 2.05                                                                           & 1.73             & 1.77  &    1.68 & 7.82   & 1.66    &    \textbf{1.62}                     & 1.63                       & 0.92\%                                  & 1.62                            \\
\textit{h.\ chr1}               & 100M/2.32                            & 2.14                                                                           & 1.78         & 1.83 &   1.74  & 7.36  &   \textbf{1.67}  &       \textbf{1.67}                         & \textbf{1.67}                       & 0.58\%                                  & 1.65                            \\
\textit{c.e.\ genome}              & 100M/2.00                              & 2.15                                                                          & 1.87         & 1.89    &  1.80  & 7.51  &  1.80   &     \textbf{1.74}                          & 1.81                       & 0.53\%                                 & 1.72                            \\
\textit{ill-quality}             & 100M/2.00                              & 0.50                                                                           & 0.35          & 0.35      & 0.34 & 6.48 &   0.34  &    \textbf{0.33}                         & 0.34                       & 2.79\%                                   & 0.51                            \\
\textit{text8}                 & 100M/4.75                             & 2.64                                                                          & 1.68        & 1.93  &  1.52  & 1.76 &  1.48   &    \textbf{1.31}                     & 1.74                                & 9.38\%                                      & 1.31                            \\
\textit{np-bases}              & 300M/2.32                              & 2.16                                                                           & 1.86               & 1.93 &  1.79 & 7.34   &   \textbf{1.70}  &      1.73                       & 1.73                       & 0.19\%                                 & 1.75                            \\
\textit{np-quality}              & 300M/6.51                             & 5.95                                                                           & 5.69     & 5.71   & 5.53 & 5.51   &   5.50  &     \textbf{5.49}                                & 5.56                       & 1.13\%                                  & 5.35                             \\ 
\textit{enwiki9}               & 500M/7.69                            & 2.72                                                                           & 1.64    & 1.94        &     1.43  & 1.66   &   1.21  &    \textbf{1.05}                    & 1.47                       & 3.67\%                                     & 1.05                            \\


\textit{num-control}               & 159.5M/8.00                            & 7.57                                                                           & 7.66    & 7.41     &   6.96   & 6.82   &   6.72  &    \textbf{6.63}                    & 6.83                 & 2.67\%                                     & 7.12                            \\
\textit{obs-spitzer}               & 198.2M/8.00                            & 6.50                                                                           & 2.51   & 2.27      &     2.20   & 2.87         &   1.73  &    \textbf{1.58}                   & 2.18                 & 6.70\%                                     & 7.74                            \\
\textit{msg-bt}               & 266.4M/8.00                            & 7.08                                                                           & 6.96     & 5.76          &    6.29   & 6.22     &   5.36  &    5.24                    & \textbf{5.21}                       & 2.08\%                                     & 6.67                            \\
\textit{audio}               & 264.6M/8.00                            & 5.75                                                                           & 4.63   &   4.98           &    4.17  & 4.92   &   3.49  &    3.44                    & \textbf{3.40}                       & 3.29\%                                     & N/A                            \\\bottomrule
\end{tabular}
\end{sc}
\end{small}

\end{table*}

==> DZip IEEETran/results_synthetic.tex <==
\begin{table*}[!htbp]
\centering
\caption{Bits per character for synthetic datasets. Best results are boldfaced. Note that 1 bpc can be achieved simply by using 1 bit per symbol for binary sequences.}
\label{table:results_synthetic}
% \vskip 0.15in
\begin{small}
\begin{sc}
\begin{tabular}{ccccccccc}
\toprule
 \textbf{Compressor} & \textit{XOR-20} & \textit{XOR-30} & \textit{XOR-50} & \textit{XOR-70}   & \textit{HMM-20} & \textit{HMM-30} & \textit{HMM-50} & \textit{HMM-70} \\ 
 \midrule
Gzip   & 1.20          & 1.20          & 1.19          & 1.19            & 1.19          & 1.19          & 1.19          & 1.19          \\ 
BSC    & 0.10          & 1.01          & 1.01          & 1.01            & 0.69          & 1.01          & 1.01          & 1.01         \\ 
7zip  & 0.05          & 0.69          & 0.65            & \textbf{0.62}          & 0.92          & 1.03          & 1.02      & 1.03          \\ 
ZPAQ   &      0.08     & 0.95          & 1.00          & 1.00            &    0.99       & 0.99          & 0.99         & \textbf{0.99}         \\
LSTM-Compress   & 4.23          & 3.19          & 4.77          & 3.43            & 3.02          & 5.19          & 3.64          & 1.01         \\ 
NNCP   &      0.125     & 0.9          & 1.00          & 1.00            &    0.57       & 1.00          & 1.00         & 1.00         \\
CMIX   &      0.02     & 0.87          & 0.93          & 0.96 &    0.50       & 0.85          & 0.99         & \textbf{0.99} \\
DZip   & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & 1.01 & \textbf{0.48} & \textbf{0.48} & \textbf{0.48} & 1.01 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table*}

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{File}     & \textbf{Len} & \textbf{Gzip} & \textbf{BSC} & \textbf{Lcom} & \textbf{Dzip} \\ \hline
% \textit{XOR20}  & 10M         &     1.20          &    0.10         &   4.23            &   \textbf{1.1e-3}            \\ \hline
% \textit{XOR30}  & 10M         &     1.20          &    1.01          &   3.19            &   \textbf{1.1e-3}            \\ \hline
% \textit{XOR40}  & 10M         &     1.19          &    1.01          &   3.22            &   \textbf{1.3e-3}            \\ \hline
% \textit{XOR50}  & 10M         &     1.19          &    1.01          &   4.77            &   \textbf{9e-4}            \\ \hline
% \textit{HMM20} & 10M         &    1.19           &   0.69           &  3.02             &  \textbf{0.47}             \\ \hline
% \textit{HMM30} & 10M         &    1.19           &    1.01          & 5.19              &   \textbf{0.47}            \\ \hline
% \textit{HMM40} & 10M         &    1.19           &    1.01          & 4.07              &   \textbf{0.47}            \\ \hline
% \textit{HMM50}    & 10M         &    1.19           &    1.01          &   3.64            &   \textbf{0.47}            \\ \hline
% \end{tabular}
% \caption{Bits per character for synthetic datasets. Best results are boldfaced.}
% \label{table:results_synthetic}
% \end{table}

==> DZip IEEETran/runningtime_table.tex <==
\begin{table*}[!htbp]
\centering
\caption{Running time of DZip in Minutes per MB for various alphabet sizes. The decoding speed with the combined model is 15\% slower than encoding. For bootstrap model the encoding and decoding speeds are similar. The bootstrap training times shown are for 8 epochs.}
\label{tab:runtime}
\vskip 0.15in
\begin{small}
\begin{sc}
\begin{tabular}{ccccccccc}
\toprule
\textbf{Step} & \textbf{$|\mathcal{S}|$=2} & \textbf{$|\mathcal{S}|$=4} & \textbf{$|\mathcal{S}|$=5} & \textbf{$|\mathcal{S}|$=27} & \textbf{$|\mathcal{S}|$=91} & \textbf{$|\mathcal{S}|$=98} & \textbf{$|\mathcal{S}|$=206} & \textbf{$|\mathcal{S}|$=256} \\ \midrule
\textit{Bootstrap Training}      & 1.5        & 2.0        & 2.0        & 5.2         & 5.2         & 5.2         & 5.5          & 5.5          \\ 
\textit{Bootstrap Encoding}     & 0.3        & 0.3        & 0.3        & 0.4         & 0.4         & 0.4         & 0.6          & 0.7          \\ 
\textit{Bootstrap Decoding}     & 0.5        & 0.5        & 0.5        & 0.7         & 0.7         & 0.7         & 0.9          & 1.1          \\ 
\textit{Combined Encoding}      & 1.9        & 2.2        & 2.2        & 2.4         & 2.4         & 2.4         & 2.7          & 2.9          \\
\textit{Combined Decoding}      & 2.0        & 2.5        & 2.5        & 2.7         & 2.7         & 2.7         & 3.0          & 3.3          \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table*}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

